InfoVisDial: An Informative Visual Dialogue Dataset by Bridging Large Multimodal and Language Models

In this paper, we build a visual dialogue dataset, named InfoVisDial, which provides rich informative answers in each round even with external knowledge related to the visual content. Different from existing datasets where the answer is compact and short, InfoVisDial contains long free-form answers with rich information in each round of dialogue. For effective data collection, the key idea is to bridge the large-scale multimodal model (e.g., GIT) and the language models (e.g., GPT-3). GIT can describe the image content even with scene text, while GPT-3 can generate informative dialogue based on the image description and appropriate prompting techniques. With such automatic pipeline, we can readily generate informative visual dialogue data at scale. Then, we ask human annotators to rate the generated dialogues to filter the low-quality conversations.Human analyses show that InfoVisDial covers informative and diverse dialogue topics: $54.4\%$ of the dialogue rounds are related to image scene texts, and $36.7\%$ require external knowledge. Each round's answer is also long and open-ended: $87.3\%$ of answers are unique with an average length of $8.9$, compared with $27.37\%$ and $2.9$ in VisDial. Last, we propose a strong baseline by adapting the GIT model for the visual dialogue task and fine-tune the model on InfoVisDial. Hopefully, our work can motivate more effort on this direction.

==> abs.tex <==
%\textbf{placeholder}
The task of visual dialog aims to build agents that can see and talk like humans, i.e., conducting fluent conversations based on the understanding of relevant visual contents. This is an important vision-language problem to study; however, the popular VisDial dataset~\cite{das2017visual} developed for this task only provides very short answers in each round of the dialogue, rendering the response less human-like. Ideally, the answer should be more free-form, 
%Pioneer studies have presented a concrete initial problem modeling of visual dialog, which retrieves a short answer in each round from a finite candidate set, conditioned on the input image, question, and dialog history. However, dialogues are open-ended in nature. The output texts should be of free-form instead of a retrieved short phrase, 
and the conversation topic can be of any visual-related content. To generate more human-like visual dialog, in this work, we propose to bridge large-scale multi-modal and language foundation models (specifically, GIT~\cite{wang2022git} and GPT-3~\cite{brown2020language}), and let them talk to each other via prompting. This process can also be understood as effectively distilling knowledge from GPT-3 to GIT. In this way, we can readily generate visual dialog data in scale. We collect dialogues based on images from the TextCap dataset, which is scene-text rich. 
To make the automatically generated data high-quality, we further use human annotators to clean and filter the dialogs. The resulting dataset is dubbed as \textbf{InfoVisDial}, as the dialogues now are more informative and content-rich. %InfoVisDial contains images from the TextCap dataset, which is scene-text rich 
%subset selected from the OpenImages dataset. 
We then finetune the pre-trained GIT model on this new dataset, and use caption and keyword accuracy metrics to evaluate the text quality and content accuracy, respectively.
Lastly, we present a detailed analysis of the dataset, providing valuable insights on the challenges of this new task.
%Furthermore, we also experiment on the VisDial dataset to evaluate the effectiveness of the proposed approach of distilling language information from the language model by finetuning the VL model. 

% We collect dialogs by prompting GPT-3 with ground-truth captions or captions generated by GIT, and using human cleaning to filter out low-quality dialogs.  



